A Non-CDCL SAT Solver with Early Conflict Detection: The Watched-Literal-Based CSFLOC Solver

CSFLOC is a non-CDCL SAT decision procedure based on counting subsumed full-length ordered clauses. The classical CSFLOC loop traverses the ordered space of full-length clauses by a monotone counter: if the current full-length clause is not subsumed by the input formula, its negation is a satisfying assignment; otherwise, a subsuming clause determines a counter jump. The main bottleneck is the repeated search for such a subsuming clause. This paper presents CSFLOC-WL, and its current implementation CSFLOC-WL3, in which this search is replaced by watched-literal prefix propagation over the negation of the current full-length clause represented by the counter. The central mechanism is early conflict detection: if propagation under a common prefix derives opposite unit consequences for the same variable, then the two reason clauses are resolved immediately and the resolvent is used as a new counter-jump cause. The resulting solver is not a CDCL solver: it has no CDCL decision tree, no restart policy, and no first-UIP backjumping loop. It remains a counter-guided full-length-clause-counting solver, but it imports the watched-literal data structure and reason clauses as engineering tools for discovering jumps. Experiments on selected UNSAT SATLIB instances compare CSFLOC-WL3 with CSFLOC21TU and CaDiCaL 3.0.0. The results are mixed: CSFLOC-WL3 is strong on several random 3-SAT instances near the random-3-SAT satisfiability threshold, whereas CSFLOC21TU remains faster on several structured cases, apparently because it contains a more mature cache mechanism that is not yet present in CSFLOC-WL3.

==> eptcsdata.tex <==
\providecommand{\firstpage}{217}
\providecommand{\publicationstatus}{M. Hospod\'ar et al. (Eds.): 17th International Conference \\on Automata and Formal Languages (AFL 2026)\\
EPTCS 451, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.451.15}{10.4204/EPTCS.451.15}}

